On a Foundation Model for Operating Systems

This paper lays down the research agenda for a domain-specific foundation model for operating systems (OSes). Our case for a foundation model revolves around the observations that several OS components such as CPU, memory, and network subsystems are interrelated and that OS traces offer the ideal dataset for a foundation model to grasp the intricacies of diverse OS components and their behavior in varying environments and workloads. We discuss a wide range of possibilities that then arise, from employing foundation models as policy agents to utilizing them as generators and predictors to assist traditional OS control algorithms. Our hope is that this paper spurs further research into OS foundation models and creating the next generation of operating systems for the evolving computing landscape.

==> tables/mdp_in_os.tex <==
%%%%%%%%%%%%% TABLE VARIABLES %%%%%%%%%%%%%
\newcommand{\TableWidthColA}{0.9cm}
\newcommand{\TableWidthColB}{1.45cm}
\newcommand{\TableWidthColC}{3.25cm}
\newcommand{\TableWidthColD}{2.25cm}
\newcommand{\TableWidthColE}{2cm}
\newcommand{\TableWidthColF}{1.75cm}
\newcommand{\TableWidthColG}{0.9cm}
\newcommand{\TableVerticalSpacing}{1.2}
%%%%%%%%%%%%% TABLE VARIABLES %%%%%%%%%%%%%

\begin{table}[h]
\setlength\tabcolsep{2.5pt}
\tiny
% \begin{adjustwidth}{-1cm}{-1cm}
\centering
\renewcommand{\arraystretch}{\TableVerticalSpacing}
\caption{MDPs of various components in the OS. \aditya{can we have a similar table for the right subtree?}}
\label{tab:mdps_in_os}
\begin{tabular}
{|p{\TableWidthColA}p{\TableWidthColB}|p{\TableWidthColC}|p{\TableWidthColD}|p{\TableWidthColE}|p{\TableWidthColF}|p{\TableWidthColG}|}
\hline
\multicolumn{2}{|c|}{\textbf{Component}} & \multicolumn{1}{c|}{\textbf{Description and Acronym}} & \multicolumn{1}{c|}{\textbf{State Space}} & \multicolumn{1}{c|}{\textbf{Action Space}} & \multicolumn{1}{c|}{\textbf{Reward}} & \multicolumn{1}{p{\TableWidthColG}|}{\textbf{Step Time}} \\ \hline
\multicolumn{1}{|p{\TableWidthColA}|}{\multirow{3}{*}{\centering {CPU}}} & \multirow{2}{*}{Scheduling} & {\bf [SCH1]:} Choose next process to run and which CPU to run it on~\cite{mllb-sigops-20} & \multirow{2}{=}{Process state(niceness, priority), Hardware state(max CPU frequency), current process-core assignment, cgroup info} & Process to core assignment, process niceness and priority values & \multirow{2}{=}{Job completion time, fairness} & ms \\ \cline{3-3} \cline{5-5} \cline{7-7} 
\multicolumn{1}{|c|}{} &  & {\bf [SCH2]:} Choosing which scheduling policy to use out of the available policies &  & Choose scheduling policy and parameters &  & sec - min \\ \cline{2-7} 
\multicolumn{1}{|c|}{} & Dynamic voltage and frequency scaling & {\bf [DVFS]:} Choosing CPU frequencies to reduce power consumptions~\cite{ztt-mobisys-21} & CPU frequency (20$\sim$30 states in between min and max) & Choose CPU frequency & CPU Performance, power consumption, temperature & sec \\ \hline
\multicolumn{1}{|p{\TableWidthColA}|}{\multirow{4}{=}{Memory Subsystem}} & Page Allocation & {\bf [PAGE1]:} What page size to use (e.g. huge pages vs normal pages) and how to allocate memory~\cite{llama-asplos-20} & Memory access patterns, Page table size & Page Size, Allocation mechanism (Buddy heap, Contiguous allocation, etc.) & Latency of memory accesses & ms \\ \cline{2-7} 
\multicolumn{1}{|c|}{} & \multirow{2}{=}{Page Replacement} & {\bf [PAGE2]:} Choose a page in the physical memory to replace with another page in virtual memory~\cite{lpr-middleware-22} & \multirow{2}{=}{Physical memory state, program instructions, page faults} & Choose the page to replace & \multirow{2}{=}{Number of page faults} & ms \\ \cline{3-3} \cline{5-5} \cline{7-7} 
\multicolumn{1}{|c|}{} &  & {\bf [PAGE3]:} Choose a page replacement algorithm &  & Choose from LRU, FIFO, MRU, Belady's &  & sec - min \\ \cline{2-7} 
\multicolumn{1}{|c|}{} & Swap Memory Management & {\bf [SWAP]:} Which processes to store on swap memory vs main memory & Process information, memory access patterns & Swap memory size, scan period, compression technique & Latency of memory accesses & sec \\ \hline
\multicolumn{1}{|p{\TableWidthColA}|}{\multirow{3}{=}{Network Subsystem}} & Packet Scheduling & {\bf [NETQUEUE]:} Order packets to send/process from the NIC queues & Past queuing delay, enqueue/dequeue rate & Packet drop rate & Throughput and delay & ms \\ \cline{2-7} 
% \multicolumn{1}{|c|}{} & Video Streaming & Generate adaptive bitrate (ABR) algorithms~\cite{pensieve-sigcomm-17} & Throughput samples, playback buffer occupancy, video chunk sizes & Bitrate decision for the next video chunk & Quality of Experience (QoE) & ms \\ \cline{2-7} 
\multicolumn{1}{|c|}{} & Congestion Control & {\bf [CC]:} Set the congestion window and pacing rate for the connection~\cite{orca-sigcomm-20,rl-icml-19,park-neurips-19} & Throughput, delay and packet loss & Congestion window and pacing rate & Throughput and delay & ms \\ \hline
\multicolumn{1}{|p{\TableWidthColA}|}{\multirow{4}{=}{Storage Subsystem}} & I/O scheduling & {\bf [IOSCH]:} Deciding in which order I/O requests should be submitted to storage devices~\cite{linnOS-osdi-20} & I/O metadata (block offset, size, read/write), queue state, historical I/O latencies & Order of I/O requests & I/O latencies & 100s of ns - ms \\ \cline{2-7} 
\multicolumn{1}{|c|}{} & Prefetching & {\bf [PREFETCH]:} Predict which segments of memory to prefetch~\cite{kml-hotstorage-21} & Past reads & Choose which segment of memory to prefetch & Throughput of future reads & 100s of ns - ms \\ \cline{2-7} 
\multicolumn{1}{|c|}{} & \multirow{2}{=}{Cache replacement} & {\bf [CACHE1]:} Decide whether to admit a new object into the cache and choose another object to evict~\cite{cachesifter-fast-22,parrot-jmlr-20,lrb-nsdi-20,glcache-fast-23} & cache object state (occupied, address, last access) & Choose a set of objects to evict/admit & Cache hit ratio & 100s of ns to ms \\ \cline{3-7} 
\multicolumn{1}{|c|}{} &  & {\bf [CACHE2]:} Choose a cache replacement algorithm to use for next time window~\cite{darwin-sigcomm-23,cacheus-fast-21} & cache object state, historical performance of caching algorithms & Choose from LRU, FIFO, MRU, GDSF, and their variants & Cache hit ratio & sec - min \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{OS}} & Host OS & {\bf [OS]:} Scheduling, Resource Management for a single host & Process states, Device states, Kernel metadata and data structures & Choose parameters, scheduling objects and resource limits & End-to-end application latencies & Few ns \\ \cline{2-7} 
\multicolumn{1}{|l|}{} & Cluster OS & {\bf [CLUSTER]:} Job scheduling and Resource management~\cite{rl-resource-alloc-icdcs-17,decima-sigcomm-19} & Job arrival patterns, Node states & Allocation jobs to nodes, preemption, provisioning & End-to-end latencies, Cluster utilisation, Fairness & ms - min \\ \hline
\end{tabular}
% \end{adjustwidth}
\end{table}


==> texfiles/discussion.tex <==
\section{Discussion}

\ds{this section would go in appendix.}
%\aditya{I would basically have a summary sentence for each para here, rename the section as conclusion and questions, and start it by saying, "We hope that our paper will generate constructive discussions at the workshop both around the high-level ideas presented above but also regarding underlying challenges such as:"}
\textbf{How do we collect data to train such a foundation model?}
A major challenge is the curation of a large dataset of OS traces.
Existing task-specific approaches only record specific features deemed relevant to the task at hand~\cite{firm-osdi-20, mllb-sigops-20, orca-sigcomm-20, linnOS-osdi-20}, while open-source traces available for some applications such as microservices ~\cite{alibaba-uservice-21}, serverless workloads~\cite{serverless-azure-20}, or cluster scheduling~\cite{borg-eurosys-15} only record the workloads and not the system state or the actions.
However, we require traces that capture a richer class of observations that help characterize the system environment and system dynamics in broader generality. Curating a single dataset that compiles data from a variety of sources in the OS is the first milestone that leads to \abbr{}. \aditya{this has been covered earlier. Drop this entire para.}

% % \todo{talk about the datasets needed and model arch. refer to the challenges spoken about in Sec 4}
% Training such a foundation model requires traces collected for different hardware specifications and for different types of applications.
% There are already lots of traces available for microservices ~\cite{alibaba-uservice-21}, serverless workloads~\cite{serverless-azure-20}, cluster scheduling~\cite{borg-eurosys-15}.
% However, these are not enough, as we also require the OS traces to capture data from different OS components and their behaviors. Further, these traces are also for cluster-level systems and not for the OS at a single host.
% Therefore, a valuable contribution to developing \abbr{} would be the collection of such a dataset, obtained by running a representative set of applications on different hardware resources and with various workloads. The works mentioned above can inform the choice of applications and workloads.
% Note that such a curation of the dataset is needed only once when pretraining \abbr{} after which only a small sample of traces would suffice for fine-tuning.~\cjr{How do we expect the foundation model to learn or encode the goodness or badness of the decisions behind a particular trace? Maybe this is something that would be obvious to ML-literati and I'm just behind. But for me, this paragraph gives me some intuition how a FM could learn what an operating system currently does, but I don't have an intuition on how traces could help it learn to do better than what it has observed.}

% \aditya{do we need a "how to train" para, where chris's question would fit in as well?}

\textbf{Why are existing LLMs/pre-trained foundation models not enough?}
Existing large language models~\cite{chowdhery2022palm, driess2023palme, llama-foundation-23} treat numbers as tokens, while all OS traces would require some numeric forms to capture hardware counters, run times, and other statistics.
Therefore, existing LLMs are unsuitable for understanding relationships between floating point numbers representing various OS-specific information, especially when the data is temporal (see~\cite{pitfalls-llm-23} for some evidence).
Instead, we seek a novel tokenizer that can use floating point numbers and also incorporate the various aspects of an OS - for example, hardware specification, concurrently running workloads, etc. \aditya{this paragraph is quite repetitive}

Further, existing LLMs are trained on a lot of data irrelevant to the OS, requiring many more parameters to train. We expect the model size for \abbr{} to be smaller than the existing LLMs, mainly because all of our tasks are specific to the OS context, and hence, the semantic space needed to be learned by the model is smaller~\cite{bloomberggpt-foundation-23}.

\textbf{What benchmarks should be used to evaluate foundation models for the OS?}
Similar to how current LLMs have various tasks to evaluate foundation models on, e.g., common sense reasoning, closed book question answering, mathematical reasoning, etc. we would need a similar set of tasks over which the performance of \abbr{} can be established. Developing such a benchmark suite would also be a crucial part of \abbr{} development. \rohit{Might be good to mention what benchmarks exist today, as a strating point. Not sure if it's exactly the same but some benchmarks do exist for CPU perf - \href{SPEC CPU2017}{https://www.spec.org/cpu2017/} - potentially, you could run the benchmark on default OS, and then on agent-driven OS and compare? I will try to find more existing benchmarks.}


\aditya{overall this section does not add much. Just make it a conclusion section and write a sentence or so about the latter two issues. First issue can be dropped.}
% \textbf{What are the risks of using \abbr{} in the OS?} \todo{pointers on what to put here?}
% \zichao{
% \begin{enumerate}
%     \item Data Bias: The efficacy of the model is significantly reliant on the distribution of its training data; thus, inputs that are out-of-distribution could lead to counterproductive or unreliable results.
%     \item Security Concerns: Employing foundation models for generating system code may introduce security vulnerabilities or loopholes.
%     \item Black-box Nature of Foundation Models: The intrinsic unexplainability of the data-driven approach in foundation models can occasionally result in contradictory predictions and fabricated outcomes, potentially causing harm to the operating system.
%     \item Data Privacy Concerns: There is a possibility that foundation models could be trained using proprietary datasets or information of a sensitive nature, which raises the risk of such information being inadvertently disclosed during deployment.
%     \item Absence of Industry Standard: Given that foundation models are a relatively new concept in the field of Operating Systems (OS), the absence of established industry standards could lead to the inefficient use of training resources and generate confusion.
% \end{enumerate}
% }

% \dk{
% Papers related to this topic:
% \begin{denseitemize}
%     \item{Training data extraction attack: "Extracting Training Data from Large Language Models" (https://www.usenix.org/system/files/sec21-carlini-extracting.pdf)}
%     \item{Use of Regex for LLM validation: "VALIDATING LARGE LANGUAGE MODELS WITH RELM"(https://arxiv.org/pdf/2211.15458.pdf)}
% \end{denseitemize}
% }

==> texfiles/finetune_llm.tex <==
\section{Finetune LLM}
Although LLMs are good for a large variety of downstream language tasks, it is limited when dealing with very domain-specific tasks such as inspecting the state of the operating system and producing policies that work well for the current workloads. Hence, it might be beneficial to finetune an LLM to adapt to our needs. Similar to \cite{driess2023palme}, we could form tasks such as 

\textit{Your current state is \textbf{S}. Give me the best policy to optimize for workload efficiency: }

Here the \textbf{S} is the encoded embedding vector of the system's state. 

==> texfiles/modeling.tex <==
% \section{Decision-making Agents in the OS}\label{sec:modeling}
\section{Learning Augmented Framework in the OS} \label{sec:modeling}
\newcommand{\states}{\handlemath{\mathcal{S}}}
\newcommand{\actions}{\handlemath{\mathcal{A}}}
\newcommand{\transition}{\handlemath{\mathcal{T}}}
\newcommand{\mdp}{\handlemath{\mathcal{M}}}

\input{tables/mdp_in_os}

\ycx{The MDP framework is more inline with the left sub-tree (agent in the loop) than the right sub-tree.}
\aditya{ Any of the tasks on the right, say an LLM generating code for an OS component, can be viewed as an MDP. I think the problem below is that the MDP definition is narrow, in that it is OS component-centric and therefore focussed on the left subtree. We need a more generic MDP definition and then map the things in the two subtrees to that definition.}

% We can consider the operating system as an agent acting within the general framework of a Markov decision process (MDP). Formally, we can define
% the OS as an agent $A$ operating over an MDP defined by the 5-tuple $(S,A,T,R,\gamma)$.
% $S$ is the state space that represents the current state of the OS environment,
% consisting of the current configurations, application workloads, and measurements
% from hardware and network interfaces. $A$ is the action space that includes all
% viable actions of the OS, such as monitoring system resources, scheduling jobs,
% and memory accesses. The action space also includes choosing the right policy from
% a set of available policies. $T = P(s_{i+1}|s_i,a_i)$ is the transition function
% that describes the probability of the agent landing in the new state $s_{i+1}$
% upon taking action $a_i$ at past state $s_i$. $R$ is the reward function and
% $\gamma$ is the discounting factor.


% Alternatively, each of the different decision-making tasks in the OS can be viewed as a
% separate sequential MDP as well. Formally, for each OS component $c$, we can define specific
% MDPs, $(S_c, A_c, T_c, R_c, \gamma_c)$ and the corresponding per-component agent
% $\mathcal{A}_c$. Prior works have also used a similar MDP formulation to come
% up with learned models for various OS tasks~\cite{park-neurips-19, whirl-sigcomm-21} \todo{add more citations}.
% Table~\ref{tab:mdps_in_os} highlights the state space, action space, and rewards for
% various per-component MDPs and for the whole OS as well. To refer to an MDP in the
% rest of the paper, we will use the corresponding acronym given in the description for
% that MDP in the table.

A significant amount of the learning augmented tasks in the OS can be formulated as an \emph{Markov Decision Process} (MDP). \aditya{warning - narrow MDP definition follows.} We start with the standard definition of an MDP $\mdp = (\states, \actions, r, \transition, \gamma)$. Here, $\states$ is the state space that represents the current state of the OS environment,
consisting of the current configurations, application workloads, and measurements
from hardware and network interfaces; $\actions$ is the action space that includes all
viable actions of the OS, such as monitoring system resources, scheduling jobs,
and memory accesses; $\transition(s' \mid s, a)$, for $s,s' \in \states$ and $a \in \actions$, is a probabilistic transition function; $r(s, a)$ for $s\in \states, a \in \actions$ is a real-valued reward function; $\lambda$ is the discounting factor.

\aditya{same issue below. it is already focused on the left subtree. In that sense, it is actually a better fit for when the left subtree is discussed.}
As shown in Table~\ref{tab:mdps_in_os}, each of the different learning-augmented tasks in the OS can be viewed as a separate MDP. Formally, for each OS component $c$, we can define specific
MDPs, $(\states_c, \actions_c, r_c, \transition_c, \gamma_c)$ and the corresponding per-component learning component. Prior works have also used a similar MDP formulation to come
up with learned models for various OS tasks~\cite{park-neurips-19, whirl-sigcomm-21} \todo{add more citations}. For these cases, FM4OS could be used for policy design (guide the policy design and use as the policy itself), transition components, or reward shaping.





